Pose Guided Person Image Generation with Hidden p-Norm Regression

In this paper, we propose a novel approach to solve the pose guided person image generation task. We assume that the relation between pose and appearance information can be described by a simple matrix operation in hidden space. Based on this assumption, our method estimates a pose-invariant feature matrix for each identity, and uses it to predict the target appearance conditioned on the target pose. The estimation process is formulated as a p-norm regression problem in hidden space. By utilizing the differentiation of the solution of this regression problem, the parameters of the whole framework can be trained in an end-to-end manner. While most previous works are only applicable to the supervised training and single-shot generation scenario, our method can be easily adapted to unsupervised training and multi-shot generation. Extensive experiments on the challenging Market-1501 dataset show that our method yields competitive performance in all the aforementioned variant scenarios.

==> related_work.tex <==
%% can be moved to first paragraph of introduction
%Generative Adversarial Networks (GANs) \cite{gan} allow computers to generate of photo-realistic images.
%GANs consist of two networks, generator and discriminator, which are jointly trained in an adversarial manner such that the discriminator cannot distinguish real images and images produced by the generator.
%This adversarial training formulation has been widely used in  pose guided person image generation task.

Pose guided person image generation has been extensively studied recently \cite{zhu2019progressive,tang2020xinggan,ren2020spatial,siarohin2018deformable}.
A major stream of works utilizes attention mechanism to model the interaction between appearance and pose information.
%pose transfer, XingGAN, 
Zhu et. al. \cite{zhu2019progressive} used a sequence of attention modules to conduct pose transfer progressively.
Tan et. al. \cite{tang2020xinggan} further improved the model capacity by introducing bidirectional appearance-pose attention.
Another type of works \cite{ren2020spatial, siarohin2018deformable} relies on deformation of hidden appearance feature map according to an affine transformation, which can be non-parametric \cite{siarohin2018deformable} or parametric \cite{ren2020spatial}.
Compared to previous works, our approach focuses on estimating a pose-invariant feature matrix, which can be easily adopted to a wide range of scenarios.

%%% TODO under determine
Our proposed pNR module is inspired by the techniques of differentiable optimization as layers \cite{amos2017optnet,agrawal2019differentiable,barratt2020least}.
These methods solve a optimization problem in the hidden space of a deep network architecture, and use the optimal solution as the input of the later part of forward process.
The differentiability of the solution enables the end-to-end training of the whole network. 
Our pNR module is a special case of these general approaches, but the solver and back-propagation of pNR module requires specific development.

%Barratt et. al. \cite{barratt2020least} proposed a method similar to pNR module,
%and used it to conduct hyper-parameter optimization task.
%However, they only considered the least square problem ($p=2$) in their method.
